Keratoconus Classifier for Smartphone-based Corneal Topographer

Keratoconus is a severe eye disease that leads to deformation of the cornea. It impacts people aged 10-25 years and is the leading cause of blindness in that demography. Corneal topography is the gold standard for keratoconus diagnosis. It is a non-invasive process performed using expensive and bulky medical devices called corneal topographers. This makes it inaccessible to large populations, especially in the Global South. Low-cost smartphone-based corneal topographers, such as SmartKC, have been proposed to make keratoconus diagnosis accessible. Similar to medical-grade topographers, SmartKC outputs curvature heatmaps and quantitative metrics that need to be evaluated by doctors for keratoconus diagnosis. An automatic scheme for evaluation of these heatmaps and quantitative values can play a crucial role in screening keratoconus in areas where doctors are not available. In this work, we propose a dual-head convolutional neural network (CNN) for classifying keratoconus on the heatmaps generated by SmartKC. Since SmartKC is a new device and only had a small dataset (114 samples), we developed a 2-stage transfer learning strategy -- using historical data collected from a medical-grade topographer and a subset of SmartKC data -- to satisfactorily train our network. This, combined with our domain-specific data augmentations, achieved a sensitivity of 91.3% and a specificity of 94.2%.

==> tables/ablations_old.tex <==
\begin{table}[h]
\centering
 \resizebox{\linewidth}{!}{
%\small
\begin{tabular}{| c | c | c | c c c|}
\toprule
 \textbf{Device} & \textbf{Fine-tuning} & \textbf{Augmentations} & \textbf{$S_e$}. & \textbf{$S_p$}. & \textbf{Score}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}

\multirow{3}{*}{SmartKC} & None & None & 88.8\% & 10.5\% & 49.7\% \\
& None & Mixup & 84.7\% & 43.1\% & 63.9\% \\
& None & Standard + Mixup & 89.1\% & 65.0\% & 77.1\% \\
& Yes & Standard + Mixup & 86.9\% & 97.1\% & 92.0\% \\
 \bottomrule
\end{tabular}
 }
\vspace{-2mm}
\caption{Ablations for fine-tuning, standard and mixup augmentations.}
% \vspace*{-3mm}
\label{tab:ablations}
\end{table}

==> tables/result_comparison_old.tex <==
\begin{table}[t]
\centering
 \resizebox{\linewidth}{!}{
%\small
\begin{tabular}{ |c | c | c | c c c|}
\toprule
 \textbf{Device} & \textbf{Input} & \textbf{Model} & \textbf{Sen}. & \textbf{Spec}. & \textbf{Score}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}

\multirow{5}{*}{Keratron} & - & PPK & 89.4\% & 94.2\% & 91.8\% \\
& SimK Feature& SVM & 78.3\% & 95.5\% & 86.9\% \\
& Axial Map & Ours: Axial branch & 92.1\% & 94.7\% & 93.4\% \\
& Tan Map & Ours: Tan branch & 92.1\% & 97.4\% & 94.8\% \\
& Axial + Tan & Ours: Combined & 94.7\% & 93.4\% & 94.1\% \\
%\vspace{2.00mm}
\hline
\multirow{4}{*}{SmartKC} & SimK Feature& SVM & 80.4\% & 100.0\% & 90.2\% \\
& Axial Map & Ours*: Axial branch & 91.3\% & 94.2\% & 92.8\% \\
& Tan Map & Ours*: Tan Branch & 86.9\% & 97.1\% & 92.0\% \\
& Axial + Tan & Ours*: Combined & 91.3\% & 94.2\% & 92.8\% \\
 \bottomrule
\end{tabular}
 }
\vspace{-2mm}
\caption{\textit{Sensitivity/Specificity of the proposed model on Keratron and \app{} data. *: is the model fine-tuned on 50\% of \app{} heatmaps in \textit{Part-2} of dataset.}}
% \vspace*{-3mm}
\label{tab:result_comparison}
\end{table}

==> tables/result_comparison_old2.tex <==
\begin{table}[t]
\centering
 \resizebox{\linewidth}{!}{
%\small
\begin{tabular}{ |c | c | c | c c c|}
\toprule
 \textbf{Device} & \textbf{Input} & \textbf{Model} & \textbf{Se} & \textbf{Sp} & \textbf{Acc.}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}

\multirow{5}{*}{Keratron} & - & PPK & 89.4\% & 94.2\% & 92.2\% \\
& sim-K feature& SVM & 78.3\% & 95.5\% & 88.6\% \\
& Axial heatmap & Ours: Axial branch & 92.1\% & 94.7\% & 93.7\% \\
& Tan heatmap & Ours: Tan branch & 92.1\% & 97.4\% & 95.3\% \\
& Axial + Tan & Ours: Combined & 94.7\% & 93.4\% & 93.9\% \\
%\vspace{2.00mm}
\hline
\multirow{4}{*}{SmartKC} & sim-K feature& SVM & 80.4\% & 100.0\% & 92.1\% \\
& Axial heatmap & Ours*: Axial branch & 91.3\% & 94.2\% & 93.1\% \\
& Tan heatmap & Ours*: Tan Branch & 86.9\% & 97.1\% & 92.9\% \\
& Axial + Tan & Ours*: Combined & 91.3\% & 94.2\% & 93.1\% \\
 \bottomrule
\end{tabular}
 }
\vspace{-2mm}
\caption{\textit{$S_e,S_p,Acc$ of the proposed model on Keratron and \app{} data. \\ *: is the model fine-tuned on 50\% heatmaps (stage-2) from \app{}-data.}}
\vspace*{-8mm}
\label{tab:result_comparison}
\end{table}
